Generative AI at Work

We study the staggered introduction of a generative AI-based conversational assistant using data from 5,172 customer support agents. Access to AI assistance increases worker productivity, as measured by issues resolved per hour, by 15\% on average, with substantial heterogeneity across workers. Less experienced and lower-skilled workers improve both the speed and quality of their output while the most experienced and highest-skilled workers see small gains in speed and small declines in quality. We also find evidence that AI assistance facilitates worker learning and improves English fluency, particularly among international agents. While AI systems improve with more training data, we find that the gains from AI adoption are largest for relatively rare problems, where human agents have less baseline training and experience. Finally, we provide evidence that AI assistance improves the experience of work along two key dimensions: customers are more polite and less likely to ask to speak to a manager.

==> preambles/header_beamer.tex <==
% Typesetting
	\usepackage{amsfonts}
	\usepackage{amssymb}
	\usepackage{amsmath}

	\usepackage{subfig}

	\usepackage{graphicx}
    
    \usepackage{multicol}
    \usepackage{tikz}
    \usetikzlibrary{calc,intersections}
    
    \usepackage{dcolumn}
    
    \usepackage{accents}
    \usepackage{adjustbox}

% Bibliography
    % \usepackage[style=authoryear-comp,natbib=true,backend=biber]{biblatex}
    % \addbibresource{Bibliography.bib}
    % \usepackage{csquotes}
	\usepackage{natbib}
 	%\bibliographystyle{apalike}
 	\bibliographystyle{aer}
	
	\usepackage{bibunits}
	\defaultbibliography{Bibliography.bib}  
	%\defaultbibliographystyle{apalike}
	\defaultbibliographystyle{aer}

	
% Links
	\usepackage{hyperref}
	\hypersetup{
    colorlinks=true,
    linkcolor=black,
    filecolor=magenta,      
    urlcolor=blue,
    citecolor = black
}
	\usepackage{cleveref}

% Todonotes
	\usepackage[framemethod=tikz]{mdframed}
	\usepackage{todonotes}
	\presetkeys{todonotes}{color=black!5,inline}{} % noline

% Boxes
    \usepackage{tcolorbox}
    \newtcbox{\feedback}{nobeforeafter,colframe=black,colback=white,boxrule=0.5pt,arc=2pt,
      boxsep=0pt,left=2pt,right=2pt,top=2pt,bottom=2pt,tcbox raise base}
      
% Theorems
    \usepackage{amsthm}
     
    \newtheorem{thm}{Theorem}
    \newtheorem{asm}{Assumption}
    \newtheorem{con}{Conjecture}
    \newtheorem{prop}{Proposition}
    \newtheorem{lem}{Lemma}
    \newtheorem{cor}{Corollary}
    \newtheorem{rem}{Remark}
    \newtheorem{defn}{Definition}

%Packages and commands for column widths in tables
\usepackage{array}
\newcolumntype{L}[1]{>{\raggedright\let\newline\\\arraybackslash}m{#1}}
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{R}[1]{>{\raggedleft\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}

%Turn off toolbar
\setbeamertemplate{navigation symbols}[default]
\beamertemplatenavigationsymbolsempty  


%Macro for wrapping text in underbrace
\usepackage{ragged2e}
\newlength\ubwidth
\newcommand\wrapunderbrace[2]{\settowidth\ubwidth{$#1$}\underbrace{#1}_{\parbox{\ubwidth}{\scriptsize\RaggedRight#2}}}


%This makes citations smaller
\makeatletter
\DeclareRobustCommand\citep
{\begingroup\footnotesize\NAT@swatrue\let\NAT@ctype\z@\NAT@partrue
    \@ifstar{\NAT@fulltrue\NAT@citetp}{\NAT@fullfalse\NAT@citetp}}
\makeatother

==> tables/15Aug2024/heterotreatment_effects.tex <==
\begin{tabular}{lcc} \hline
 & (1) & (2) \\
VARIABLES & Pre-AI Skill & Pre-AI Tenure \\ \hline
 &  &  \\
Q1 (Lowest Skilled) & 0.527*** &  \\
 & (0.0487) &  \\
Q2 & 0.315*** &  \\
 & (0.0562) &  \\
Q3 & 0.302*** &  \\
 & (0.0435) &  \\
Q4 & 0.261*** &  \\
 & (0.0545) &  \\
Q5 (Highest Skilled) & 0.0154 &  \\
 & (0.0646) &  \\
<1 Mos. &  & 0.707*** \\
 &  & (0.0665) \\
1-2 Mos. &  & 0.388*** \\
 &  & (0.0422) \\
3-6 Mos. &  & 0.361*** \\
 &  & (0.0665) \\
7-12 Mos. &  & 0.337*** \\
 &  & (0.0537) \\
>12 Mos. &  & 0.0276 \\
 &  & (0.0594) \\
 &  &  \\
Observations & 12,295 & 8,148 \\
R-squared & 0.580 & 0.536 \\
Year Month FE & Yes & Yes \\
Location FE & Yes & Yes \\
Agent FE & Yes & Yes \\
Agent Tenure FE & Yes & No \\
Agent Skill at AI FE & No & Yes \\
 DV Mean & 1.727 & 1.727 \\ \hline
\multicolumn{3}{c}{ Robust standard errors in parentheses} \\
\multicolumn{3}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.10} \\
\end{tabular}


==> tables/15Aug2024/ivdd_companyteam.tex <==
\begin{tabular}{lcccccc} \hline
 & (1) & (2) & (3) & (4) & (5) & (6) \\
VARIABLES & Individual Treatment & Res./Hr & AHT & Chats/Hr & Res. Rate & NPS \\ \hline
 &  &  &  &  &  &  \\
Earliest Team Treatment & 0.311*** &  &  &  &  &  \\
 & (0.0163) &  &  &  &  &  \\
Post AI X Individual Treatment &  & 0.550*** & -3.622** & 0.412*** & 0.0740*** & -0.518 \\
 &  & (0.0943) & (1.444) & (0.0791) & (0.0184) & (0.946) \\
 &  &  &  &  &  &  \\
Observations & 21,839 & 12,295 & 21,839 & 21,839 & 12,295 & 12,541 \\
R-squared & 0.813 & 0.177 & 0.102 & 0.115 & 0.007 & 0.007 \\
Year Month FE & YES & YES & YES & YES & YES & YES \\
Location FE & YES & YES & YES & YES & YES & YES \\
Agent FE & YES & YES & YES & YES & YES & YES \\
Agent Tenure FE & YES & YES & YES & YES & YES & YES \\
 Number of agent\_id &  & 2,163 & 3,633 & 3,633 & 2,163 & 2,214 \\ \hline
\multicolumn{7}{c}{ Robust standard errors in parentheses} \\
\multicolumn{7}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.10} \\
\end{tabular}


==> tables/15Aug2024/outages_table.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{l}}
\toprule
                &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
                &\multicolumn{1}{c}{Non Outage}&\multicolumn{1}{c}{AI Outages}&\multicolumn{1}{c}{Outages - High Receptivity}&\multicolumn{1}{c}{Outages - Low Receptivity}\\
\midrule
lead30          &0.578         &1.661\sym{**} &3.423\sym{***}&-2.089         \\
                &(0.718)         &(0.791)         &(1.189)         &(3.104)         \\
\addlinespace
lead29          &0.987         &2.229\sym{**} &3.414\sym{**} &-0.716         \\
                &(0.845)         &(0.878)         &(1.437)         &(3.099)         \\
\addlinespace
lead28          &0.981         &2.051\sym{**} &3.429\sym{**} &-0.525         \\
                &(0.844)         &(0.883)         &(1.482)         &(3.156)         \\
\addlinespace
lead27          &0.214         &1.379         &3.394\sym{**} &-1.792         \\
                &(0.816)         &(0.856)         &(1.391)         &(2.997)         \\
\addlinespace
lead26          &-0.627         &0.510         &2.806\sym{**} &-3.376         \\
                &(0.779)         &(0.821)         &(1.427)         &(2.766)         \\
\addlinespace
lead25          &-0.818         &0.354         &2.715\sym{**} &-4.009         \\
                &(0.707)         &(0.751)         &(1.219)         &(2.668)         \\
\addlinespace
lead24          &-1.291\sym{*}  &-0.018         &1.099         &-4.471\sym{*}  \\
                &(0.765)         &(0.812)         &(1.287)         &(2.640)         \\
\addlinespace
lead23          &-2.339\sym{***}&-1.077         &0.497         &-5.814\sym{**} \\
                &(0.712)         &(0.754)         &(1.284)         &(2.591)         \\
\addlinespace
lead22          &-1.778\sym{**} &-0.490         &1.970         &-5.063\sym{**} \\
                &(0.697)         &(0.733)         &(1.303)         &(2.502)         \\
\addlinespace
lead21          &-1.611\sym{**} &-0.299         &1.437         &-5.000\sym{**} \\
                &(0.663)         &(0.698)         &(1.215)         &(2.336)         \\
\addlinespace
lead20          &-1.518\sym{**} &-0.119         &2.819\sym{**} &-5.187\sym{**} \\
                &(0.674)         &(0.703)         &(1.266)         &(2.283)         \\
\addlinespace
lead10          &0.684         &2.085\sym{***}&3.391\sym{***}&0.284         \\
                &(0.550)         &(0.581)         &(0.880)         &(1.590)         \\
\addlinespace
lead9           &0.549         &2.126\sym{***}&4.056\sym{***}&1.003         \\
                &(0.529)         &(0.551)         &(0.890)         &(1.388)         \\
\addlinespace
lead8           &-0.222         &1.410\sym{***}&3.239\sym{***}&0.340         \\
                &(0.479)         &(0.504)         &(0.771)         &(1.299)         \\
\addlinespace
lead7           &-0.302         &1.267\sym{***}&2.354\sym{***}&1.025         \\
                &(0.470)         &(0.486)         &(0.798)         &(1.141)         \\
\addlinespace
lead6           &0.874\sym{*}  &2.204\sym{***}&4.081\sym{***}&2.210\sym{**} \\
                &(0.463)         &(0.468)         &(0.786)         &(1.079)         \\
\addlinespace
lead5           &0.439         &1.444\sym{***}&2.953\sym{***}&1.736\sym{*}  \\
                &(0.389)         &(0.378)         &(0.591)         &(0.885)         \\
\addlinespace
lead4           &0.415         &1.052\sym{***}&2.222\sym{***}&1.258\sym{*}  \\
                &(0.336)         &(0.321)         &(0.471)         &(0.703)         \\
\addlinespace
lead3           &0.135         &0.343         &1.314\sym{***}&0.218         \\
                &(0.305)         &(0.297)         &(0.482)         &(0.627)         \\
\addlinespace
lead2           &-0.146         &-0.209         &0.723\sym{*}  &-0.869\sym{*}  \\
                &(0.248)         &(0.247)         &(0.411)         &(0.469)         \\
\addlinespace
lag0            &-4.105\sym{***}&-3.471         &-5.236         &9.410\sym{***}\\
                &(0.270)         &(3.713)         &(3.732)         &(3.564)         \\
\addlinespace
lag1            &-4.523\sym{***}&-2.420         &-6.699\sym{*}  &0.000         \\
                &(0.313)         &(3.242)         &(4.052)         &(.)         \\
\addlinespace
lag2            &-4.785\sym{***}&0.767         &-0.201         &0.000         \\
                &(0.335)         &(3.112)         &(3.858)         &(.)         \\
\addlinespace
lag3            &-4.424\sym{***}&-2.851         &-2.677         &6.005         \\
                &(0.333)         &(2.663)         &(3.915)         &(4.099)         \\
\addlinespace
lag4            &-4.225\sym{***}&-2.423\sym{*}  &-4.011\sym{**} &4.851         \\
                &(0.350)         &(1.442)         &(2.015)         &(3.663)         \\
\addlinespace
lag5            &-4.084\sym{***}&0.838         &0.695         &7.871         \\
                &(0.380)         &(1.744)         &(2.042)         &(5.904)         \\
\addlinespace
lag6            &-4.300\sym{***}&-7.799\sym{***}&-8.574\sym{***}&-2.303         \\
                &(0.388)         &(1.836)         &(2.168)         &(3.167)         \\
\addlinespace
lag7            &-4.445\sym{***}&-8.494\sym{***}&-9.532\sym{***}&-2.161         \\
                &(0.393)         &(1.635)         &(1.687)         &(3.209)         \\
\addlinespace
lag8            &-3.804\sym{***}&-4.672\sym{*}  &-2.163         &-8.059\sym{***}\\
                &(0.411)         &(2.647)         &(2.471)         &(3.023)         \\
\addlinespace
lag9            &-3.628\sym{***}&-8.705\sym{***}&-8.842\sym{***}&0.318         \\
                &(0.440)         &(1.660)         &(1.930)         &(5.166)         \\
\addlinespace
lag10           &-3.609\sym{***}&-4.386\sym{**} &-4.486\sym{**} &-0.233         \\
                &(0.501)         &(1.720)         &(2.040)         &(4.273)         \\
\addlinespace
lag11           &-3.305\sym{***}&-2.779\sym{**} &-6.857\sym{**} &0.539         \\
                &(0.486)         &(1.380)         &(3.252)         &(4.003)         \\
\addlinespace
lag12           &-3.479\sym{***}&-1.966         &-4.630         &-8.939\sym{**} \\
                &(0.517)         &(3.003)         &(4.248)         &(3.510)         \\
\addlinespace
lag13           &-3.458\sym{***}&-1.636         &-2.437         &-3.302         \\
                &(0.534)         &(1.195)         &(1.899)         &(3.779)         \\
\addlinespace
lag14           &-3.236\sym{***}&-5.619\sym{***}&-6.189\sym{**} &-11.504\sym{**} \\
                &(0.544)         &(1.935)         &(3.044)         &(5.232)         \\
\addlinespace
lag15           &-3.741\sym{***}&-2.329         &-3.526         &-0.599         \\
                &(0.587)         &(1.530)         &(2.219)         &(3.999)         \\
\addlinespace
lag16           &-3.498\sym{***}&-5.178\sym{***}&-7.259\sym{**} &-0.798         \\
                &(0.585)         &(1.484)         &(2.862)         &(4.363)         \\
\addlinespace
lag17           &-4.128\sym{***}&-6.336\sym{***}&-8.646\sym{***}&-4.976         \\
                &(0.595)         &(1.518)         &(2.370)         &(4.169)         \\
\addlinespace
lag18           &-4.200\sym{***}&-6.829\sym{***}&-8.894\sym{**} &-4.711         \\
                &(0.580)         &(1.321)         &(3.632)         &(3.947)         \\
\addlinespace
lag19           &-4.100\sym{***}&-5.555\sym{***}&-3.135         &-3.573         \\
                &(0.676)         &(1.509)         &(3.145)         &(4.125)         \\
\addlinespace
lag20           &-4.096\sym{***}&-3.042\sym{**} &-3.776\sym{*}  &-0.282         \\
                &(0.619)         &(1.316)         &(2.126)         &(4.593)         \\
\midrule
Year Month FE   &Yes         &Yes         &Yes         &Yes         \\
Agent FE        &Yes         &Yes         &Yes         &Yes         \\
Agent Tenure FE &Yes         &Yes         &Yes         &Yes         \\
DV Mean         &41.982         &41.982         &41.982         &41.982         \\
R-squared       &.12         &.104         &.113         &.083         \\
Observations    &2,969,371         &1,829,527         &1,220,852         &323,810         \\
\bottomrule
\multicolumn{5}{l}{\footnotesize Standard errors in parentheses}\\
\multicolumn{5}{l}{\footnotesize \sym{*} \(p<0.10\), \sym{**} \(p<0.05\), \sym{***} \(p<0.01\)}\\
\end{tabular}
}


==> tables/17Apr2023/AlternativeDiD.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{cccc}}
\hline\hline
                &\shortstack{Point\\Estimate}&\shortstack{Standard\\Error}&\shortstack{Lower Bound\\ 95\% Confidence\\Interval}&\shortstack{Upper Bound\\ 95\% Confidence\\Interval}\\
\hline
TWFE-OLS        &    0.137&    0.014&    0.108&    0.165\\
Borusyak-Jaravel-Spiess&    0.257&    0.028&    0.203&    0.311\\
Callaway-Sant'Anna&    0.239&    0.025&    0.189&    0.289\\
DeChaisemartin-D'Haultfeuille&    0.116&    0.021&    0.075&    0.156\\
Sun-Abraham     &    0.237&    0.037&    0.165&    0.308\\
\hline\hline
\end{tabular}
}


==> tables/17Apr2023/AlternativeDiD_lnrph_cresta.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{cccc}}
\hline\hline
                &\shortstack{Point\\Estimate}&\shortstack{Standard\\Error}&\shortstack{Lower Bound\\ 95\% Confidence\\Interval}&\shortstack{Upper Bound\\ 95\% Confidence\\Interval}\\
\hline
TWFE-OLS        &    0.137&    0.014&    0.108&    0.165\\
Borusyak-Jaravel-Spiess&    0.257&    0.028&    0.203&    0.311\\
Callaway-Sant'Anna&    0.239&    0.025&    0.189&    0.289\\
DeChaisemartin-D'Haultfoeuille&    0.116&    0.021&    0.075&    0.156\\
Sun-Abraham     &    0.237&    0.037&    0.165&    0.308\\
\hline\hline
\end{tabular}
}


==> tables/24June2024/adoptionr2_formatted.tex <==
\begin{tabular}{lccc} \hline
 & (1) & (2) & (3) \\
VARIABLES & Ever Treated & Ever Treated & Ever Treated \\ \hline
Adjusted R2 & 0.0754 & 0.195 & 0.576 \\
Observations & 23,378 & 23,377 & 23,369 \\
Company FE & YES &  &  \\
Company-Location FE &  & YES &  \\
 Company-Location-Team FE &  &  & YES \\ \hline
\multicolumn{4}{c}{ Standard errors in parentheses} \\
\multicolumn{4}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.1} \\
\end{tabular}


==> tables/24June2024/attrition.tex <==
\begin{tabular}{lcccc} \hline
 & (1) & (2) & (3) & (4) \\
VARIABLES & Leaves this Month & Leaves this Month & Leaves this Month & Leaves this Month \\ \hline
 &  &  &  &  \\
0 Mos. &  & -0.0952** &  &  \\
 &  & (0.0342) &  &  \\
1-2 Mos. &  & -0.121*** &  &  \\
 &  & (0.0341) &  &  \\
A3-6 Mos. &  & -0.0850*** &  &  \\
 &  & (0.0285) &  &  \\
7-12 Mos. &  & -0.0803* &  &  \\
 &  & (0.0437) &  &  \\
>12 Mos. &  & -0.0306 &  &  \\
 &  & (0.0546) &  &  \\
Post AI X Ever Treated & -0.0868** &  &  &  \\
 & (0.0319) &  &  &  \\
AI X Q1 (Low) &  &  & -0.0655*** &  \\
 &  &  & (0.0189) &  \\
AI X Q2 &  &  & -0.0864*** &  \\
 &  &  & (0.0175) &  \\
AI X Q3 &  &  & -0.0741*** &  \\
 &  &  & (0.0184) &  \\
AI X Q4 &  &  & -0.0936*** &  \\
 &  &  & (0.0147) &  \\
AI X Q5 (High) &  &  & -0.0531* &  \\
 &  &  & (0.0277) &  \\
AI X US &  &  &  & -0.156** \\
 &  &  &  & (0.0580) \\
AI X non US &  &  &  & -0.0826** \\
 &  &  &  & (0.0338) \\
AI X Remote &  &  &  & -0.0368*** \\
 &  &  &  & (0.0113) \\
 &  &  &  &  \\
Observations & 17,902 & 17,902 & 17,902 & 17,902 \\
R-squared & 0.206 & 0.206 & 0.206 & 0.206 \\
Year Month FE & YES & YES & YES & YES \\
Location FE & YES & YES & YES & YES \\
Agent Tenure FE & YES & YES & YES & YES \\
DV Mean & 0.288 & 0.288 & 0.288 & 0.288 \\
 Agent Location FE &  & YES & YES & YES \\ \hline
\multicolumn{5}{c}{ Robust standard errors in parentheses} \\
\multicolumn{5}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.10} \\
\end{tabular}


==> tables/24June2024/balance_table.tex <==
\begin{tabular}{l*{3}c}
\toprule
 & (1) & (2) & (3) \\
Variable & Control & Treatment & Difference \\
\midrule
AHT&35.761&35.299&-0.462***\\
&(13.503)&(13.468)&(0.000)\\
Resolution Rate&0.800&0.833&0.033***\\
&(0.203)&(0.146)&(0.000)\\
Customer Satisfaction&75.566&78.679&3.113***\\
&(19.864)&(14.327)&(0.000)\\
Res. per Hour&2.097&2.257&0.160***\\
&(0.809)&(0.703)&(0.000)\\
\midrule
Observations & 944,848 & 881,101 & 1,825,949 \\
\bottomrule
\end{tabular}


==> tables/24June2024/ivdd_companyloc.tex <==
\begin{tabular}{lcccccc} \hline
 & (1) & (2) & (3) & (4) & (5) & (6) \\
VARIABLES & Post AI X Individual Treatment & Res./Hr & AHT & Chats/Hr & Res. Rate & NPS \\ \hline
 &  &  &  &  &  &  \\
Post AI X Group Treatment & 0.0870*** &  &  &  &  &  \\
 & (0.0278) &  &  &  &  &  \\
Post AI X Individual Treatment &  & -7.815 & -14.69 & 0.0379 & 0.808 & -109.1 \\
 &  & (169.3) & (11.53) & (0.484) & (14.64) & (732.7) \\
 &  &  &  &  &  &  \\
Observations & 21,839 & 12,295 & 21,839 & 21,839 & 12,295 & 12,541 \\
R-squared & 0.796 & -10.191 & 0.015 & 0.094 & -1.419 & -8.535 \\
Year Month FE & YES & YES & YES & YES & YES & YES \\
Location FE & YES & YES & YES & YES & YES & YES \\
Agent FE & YES & YES & YES & YES & YES & YES \\
Agent Tenure FE & YES & YES & YES & YES & YES & YES \\
 Number of agent\_id &  & 2,163 & 3,633 & 3,633 & 2,163 & 2,214 \\ \hline
\multicolumn{7}{c}{ Robust standard errors in parentheses} \\
\multicolumn{7}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.10} \\
\end{tabular}


==> tables/24June2024/ivdd_companylocteam.tex <==
\begin{tabular}{lcccccc} \hline
 & (1) & (2) & (3) & (4) & (5) & (6) \\
VARIABLES & Individual Treatment & Res./Hr & AHT & Chats/Hr & Res. Rate & NPS \\ \hline
 &  &  &  &  &  &  \\
Earliest Team Treatment & 0.311*** &  &  &  &  &  \\
 & (0.0163) &  &  &  &  &  \\
Post AI X Individual Treatment &  & 0.550*** & -3.622** & 0.412*** & 0.0740*** & -0.518 \\
 &  & (0.0943) & (1.444) & (0.0791) & (0.0184) & (0.946) \\
 &  &  &  &  &  &  \\
Observations & 21,839 & 12,295 & 21,839 & 21,839 & 12,295 & 12,541 \\
R-squared & 0.813 & 0.177 & 0.102 & 0.115 & 0.007 & 0.007 \\
Year Month FE & YES & YES & YES & YES & YES & YES \\
Location FE & YES & YES & YES & YES & YES & YES \\
Agent FE & YES & YES & YES & YES & YES & YES \\
Agent Tenure FE & YES & YES & YES & YES & YES & YES \\
 Number of agent\_id &  & 2,163 & 3,633 & 3,633 & 2,163 & 2,214 \\ \hline
\multicolumn{7}{c}{ Robust standard errors in parentheses} \\
\multicolumn{7}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.10} \\
\end{tabular}


==> tables/24June2024/ivdd_companyteam.tex <==
\begin{tabular}{lcccccc} \hline
 & (1) & (2) & (3) & (4) & (5) & (6) \\
VARIABLES & Individual Treatment & Res./Hr & AHT & Chats/Hr & Res. Rate & NPS \\ \hline
 &  &  &  &  &  &  \\
Earliest Team Treatment & 0.311*** &  &  &  &  &  \\
 & (0.0163) &  &  &  &  &  \\
Post AI X Individual Treatment &  & 0.550*** & -3.622** & 0.412*** & 0.0740*** & -0.518 \\
 &  & (0.0943) & (1.444) & (0.0791) & (0.0184) & (0.946) \\
 &  &  &  &  &  &  \\
Observations & 21,839 & 12,295 & 21,839 & 21,839 & 12,295 & 12,541 \\
R-squared & 0.813 & 0.177 & 0.102 & 0.115 & 0.007 & 0.007 \\
Year Month FE & YES & YES & YES & YES & YES & YES \\
Location FE & YES & YES & YES & YES & YES & YES \\
Agent FE & YES & YES & YES & YES & YES & YES \\
Agent Tenure FE & YES & YES & YES & YES & YES & YES \\
 Number of agent\_id &  & 2,163 & 3,633 & 3,633 & 2,163 & 2,214 \\ \hline
\multicolumn{7}{c}{ Robust standard errors in parentheses} \\
\multicolumn{7}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.10} \\
\end{tabular}


==> tables/24June2024/maindd_others.tex <==
\begin{tabular}{lcccc} \hline
 & (1) & (2) & (3) & (4) \\
VARIABLES & AHT & Chats/Hr & Res. Rate & NPS \\ \hline
 &  &  &  &  \\
Post AI X Ever Treated & -3.746*** & 0.365*** & 0.0132* & -0.119 \\
 & (0.476) & (0.0364) & (0.00706) & (0.659) \\
 &  &  &  &  \\
Observations & 21,839 & 21,839 & 12,295 & 12,541 \\
R-squared & 0.591 & 0.563 & 0.371 & 0.526 \\
Year Month FE & Yes & Yes & Yes & Yes \\
Location FE & Yes & Yes & Yes & Yes \\
Agent FE & Yes & Yes & Yes & Yes \\
Agent Tenure & Yes & Yes & Yes & Yes \\
 DV Mean & 40.64 & 2.559 & 0.822 & 79.59 \\ \hline
\multicolumn{5}{c}{ Robust standard errors in parentheses} \\
\multicolumn{5}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.10} \\
\end{tabular}


==> tables/24June2024/maindd_rph.tex <==
\begin{tabular}{lccc} \hline
 & (1) & (2) & (3) \\
VARIABLES & Resolutions/Hr & Resolutions/Hr & Resolutions/Hr \\ \hline
 &  &  &  \\
Post AI X Ever Treated & 0.469*** & 0.371*** & 0.301*** \\
 & (0.0542) & (0.0519) & (0.0498) \\
Ever Treated & 0.110* &  &  \\
 & (0.0589) &  &  \\
 &  &  &  \\
Observations & 13,192 & 12,295 & 12,295 \\
R-squared & 0.249 & 0.562 & 0.575 \\
Year Month FE & Yes & Yes & Yes \\
Location FE & Yes & Yes & Yes \\
Agent FE & - & Yes & Yes \\
Agent Tenure & - & - & Yes \\
 DV Mean & 2.123 & 2.176 & 2.176 \\ \hline
\multicolumn{4}{c}{ Robust standard errors in parentheses} \\
\multicolumn{4}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.10} \\
\end{tabular}


==> tables/24June2024/rctdd.tex <==
\begin{tabular}{lccccc} \hline
 & (1) & (2) & (3) & (4) & (5) \\
VARIABLES & Res./Hr & AHT & Chats/Hr & Res. Rate & NPS \\ \hline
 &  &  &  &  &  \\
Post AI X Ever Treated & 0.202** & -3.713*** & 0.105 & 0.0169 & -1.393 \\
 & (0.0850) & (1.045) & (0.0718) & (0.0246) & (1.529) \\
 &  &  &  &  &  \\
Observations & 6,998 & 15,100 & 15,100 & 6,998 & 7,176 \\
R-squared & 0.568 & 0.574 & 0.566 & 0.383 & 0.517 \\
Year Month FE & Yes & Yes & Yes & Yes & Yes \\
Location FE & Yes & Yes & Yes & Yes & Yes \\
Agent FE & Yes & Yes & Yes & Yes & Yes \\
Agent Tenure & Yes & Yes & Yes & Yes & Yes \\
 DV Mean & 1.956 & 43 & 2.378 & 0.808 & 79.68 \\ \hline
\multicolumn{6}{c}{ Robust standard errors in parentheses} \\
\multicolumn{6}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.10} \\
\end{tabular}


==> tables/24June2024/robustdd_nchat_weight.tex <==
\begin{tabular}{lccccc} \hline
 & (1) & (2) & (3) & (4) & (5) \\
VARIABLES & Res./Hour & AHT & Chats/Hr & Res. Rate & NPS \\ \hline
 &  &  &  &  &  \\
Post AI X Ever Treated & 0.252*** & -3.100*** & 0.295*** & 0.00325 & -0.119 \\
 & (0.0505) & (0.514) & (0.0404) & (0.00549) & (0.659) \\
 &  &  &  &  &  \\
Observations & 12,295 & 21,839 & 21,839 & 12,295 & 12,541 \\
R-squared & 0.650 & 0.756 & 0.721 & 0.465 & 0.526 \\
Year Month FE & Yes & Yes & Yes & Yes & Yes \\
Location FE & Yes & Yes & Yes & Yes & Yes \\
Agent FE & Yes & Yes & Yes & Yes & Yes \\
Agent Tenure & Yes & Yes & Yes & Yes & Yes \\
 DV Mean & 2.457 & 38.66 & 2.886 & 0.839 & 79.59 \\ \hline
\multicolumn{6}{c}{ Robust standard errors in parentheses} \\
\multicolumn{6}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.10} \\
\end{tabular}


==> tables/24June2024/robustness_clustering.tex <==
\begin{tabular}{lccc} \hline
 & (1) & (2) & (3) \\
Level of Clustering & Individual & Location & Location Team \\ \hline
 &  &  &  \\
Post AI X Ever Treated & 0.301*** & 0.301*** & 0.301*** \\
 & (0.0329) & (0.0498) & (0.0453) \\
 &  &  &  \\
Observations & 12,295 & 12,295 & 12,295 \\
R-squared & 0.575 & 0.575 & 0.575 \\
Year Month FE & Yes & Yes & Yes \\
Location FE & Yes & Yes & Yes \\
Agent FE & Yes & Yes & Yes \\
Agent Tenure & Yes & Yes & Yes \\
 DV Mean & 2.176 & 2.176 & 2.176 \\ \hline
\multicolumn{4}{c}{ Robust standard errors in parentheses} \\
\multicolumn{4}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.10} \\
\end{tabular}


==> tables/24June2024/sentiment.tex <==
\begin{tabular}{lcc} \hline
 & (1) & (2) \\
VARIABLES & Mean(Customer Sentiment) & Mean(Agent Sentiment) \\ \hline
 &  &  \\
Post AI X Ever Treated & 0.177*** & 0.0198*** \\
 & (0.0133) & (0.00315) \\
 &  &  \\
Observations & 21,218 & 21,218 \\
R-squared & 0.485 & 0.596 \\
Year Month FE & YES & YES \\
Location FE & YES & YES \\
Agent FE & YES & YES \\
Agent Tenure FE & YES & YES \\
 DV Mean & 0.141 & 0.896 \\ \hline
\multicolumn{3}{c}{ Robust standard errors in parentheses} \\
\multicolumn{3}{c}{ *** p$<$0.01, ** p$<$0.05, * p$<$0.10} \\
\end{tabular}

